Optimal Policies for Recovery of Multiple Systems After Disruptions

We consider a scenario where a system experiences a disruption, and the states (representing health values) of its components continue to reduce over time, unless they are acted upon by a controller. Given this dynamical setting, we consider the problem of finding an optimal control (or switching) sequence to maximize the sum of the weights of the components whose states are brought back to the maximum value. We first provide several characteristics of the optimal policy for the general (fully heterogeneous) version of this problem. We then show that under certain conditions on the rates of repair and deterioration, we can explicitly characterize the optimal control policy as a function of the states. When the deterioration rate (when not being repaired) is larger than or equal to the repair rate, and the deterioration and repair rates as well as the weights are homogeneous across all the components, the optimal control policy is to target the component that has the largest state value at each time step. On the other hand, if the repair rates are sufficiently larger than the deterioration rates, the optimal control policy is to target the component whose state minus the deterioration rate is least in a particular subset of components at each time step.

==> introduction_old.tex <==
\section{Introduction}
We study a control problem where the states (or healths) of various components of a system continue to reduce when not being controlled until the states reach a threshold termed as \textit{permanent failure} state. A controller or an entity is responsible for increasing the states of components to another threshold termed as the \textit{full health} or \textit{permanent repair} state. We consider the scenario after a system faces disruption or shock such that the initial states of the components lie in between the \textit{permanent repair} or \textit{permanent failure} states and the states of components do not change once they reach either of the two thresholds. Under these dynamics, the entity needs to make optimal control decisions of increasing the states of different components to maximize a performance criterion or reward, for e.g., maximizing the number of components that reach the full health state. We aim to study this dynamical problem through a control-theoretic framework. This problem has applications in multiple areas like post-disaster recovery, protection of cyber-physical systems against multiple attacks, fire fighting, epidemic control etc. For instance, after disasters infrastructure components face accelerated deterioration due to processes such as floods and corrosion \cite{gaspard2007impact}, and because of that they can deteriorate to such a level that they become unusable and require full replacement, which is expensive and thus undesirable. Similarly, when multiple computer servers get partially damaged by a virus/malware, the protecting agency would face a limited amount of time before the servers become fully damaged. Likewise, the objective of the fire-fighters is to ensure a fire does not enters the state of \textit{flashover}, which represents the fully developed stage at which there is hardly any hope of saving a property or an individual \cite{metropolitan2009fire}. Therefore, shortage of the available manpower and resources can compel the fire fighters to make optimal control decisions while facing simultaneous fires located in different regions \cite{smeby2013fire}. 

Our problem comes under the general class of optimal control and scheduling of switched systems \cite{zhang2009value,gorges2010optimal}, which are a type of hybrid systems \cite{borrelli2005dynamic,bemporad2006logic}. A switched system consists of multiple subsystems that are governed by different dynamical rules such that only one subsystem is active at one point of time. In our problem, a subsystem is governed by the component whose state is increased by the entity at a particular time step (and it also depends on whether the states of components are at either of the two thresholds). Since the entity periodically decides to increase the states of components at a fixed time interval, our problem comes under the class of discrete-time switched systems. The main source of complexity in the optimal control and scheduling of discrete-time switched systems is the combinatorial number of feasible switching sequences \cite{bemporad2006logic}. In the past decade, there have been some advancements in theoretical results and computational frameworks for solving switched systems. The papers \cite{zhang2009value,gorges2010optimal} characterize optimal/near-optimal control policies for discrete-time switched linear systems but with linear or quadratic cost/reward functions. However, there are no theoretical results or computational frameworks that efficiently solve the optimal control problems for all types of switched systems and most results are formulation dependent \cite{zhu2015optimal}. Therefore, optimal control and scheduling of switched systems remains an area of active research. 

% A disaster is a non-routine event that has the potential for catastrophic impacts on physical, natural and social systems. For instance, Hurricane Sandy caused 147 direct casualties along its path and brought damage in excess of \$50 billion in the United States \cite{blake2013tropical}. The recovery of infrastructure after a disaster is a massive task which, in turn, also affects the return patterns of displaced communities. It is therefore imperative for emergency-response agencies to determine an optimal sequence to repair the damaged components of physical infrastructure in order to maximize recovery. 
% * <sukkusur@purdue.edu> 2018-12-21T15:53:14.226Z:
% 
% Cite a reference for this and the community level variables.
% 
% ^.

% There are various studies that involve sequencing of recovery decisions in post-disaster scenarios. Some studies develop network flow-based models for physical infrastructure networks where maximizing flow is considered equivalent to maximizing recovery \cite{nurre2012restoring}. Studies in operations research have focused on finding an optimal sequence of targeting different roads in order to remove debris after disasters \cite{ccelik2015post}. However, these studies mainly focus on recovery of individual elements belonging to a certain type of physical infrastructure (e.g., roads in a transportation network) rather than focusing on sequencing decisions for repairing portions of physical infrastructure with varying damage/health levels. Furthermore, these studies do not model deterioration of physical infrastructure over time if a component is not being repaired. Such deterioration is commonly observed in real-world post-disaster scenarios; for example road infrastructure deteriorates over time in flooded areas after hurricanes \cite{gaspard2007impact}. 

% Our paper considers the problem of finding an optimal sequence (or control policy) that a recovery agency/entity should follow in order to maximize the number of  physical infrastructure components that are returned to full health. Specifically, we consider scenarios where the health of a component decreases over time (at a certain rate) if it is not being repaired, and increases (also at a given rate) during those time-steps when it is being repaired.  
The reward function in our control problem is the weighted number of components that can be fixed to full health and therefore it is not a linear or a quadratic function. We find that optimal control policies are feedback policies that depend on the relationship between the rates of increase and decrease of states. Specifically, the contributions of this paper are as follows: 1) we prove that the optimal control policy is to increase the state of a component to full health before the entity switches to increase the state of another component when the decrease rates are larger than the corresponding increase rates; 2) we show that the optimal control policy is to target the component that has the largest state at each time step when the decrease and increase rates as well as the weights of components are homogeneous across all the components and the decrease rates are larger than the increase rates; and 3) we prove that the optimal control policy is to target the component that has the least value of state minus the rate of decrease in a particular subset of components at each time step when the rates of increase are sufficiently larger than the corresponding rates of decrease. 

\section{Relationship with the existing literature}
At a high level, another type of switched systems control problems such as scheduling of thermostatically controlled loads \cite{nghiem2011green,nilsson2017class} also has similarities to our problem. These studies characterize scheduling control policies so that states  (e.g., temperature) of the components (e.g., room) in the system always stay in a given interval.  %\cite{nghiem2011green} characterize a \textit{lazy} scheduling policy where switching decisions are only made when the state of a component reaches either of the interval thresholds. This policy is not optimal as states of some components may violate thresholds if the states of too many components simultaneously reach a threshold. \cite{nilsson2017class} characterize an optimal policy in which the components that are closest to the threshold values are switched, given some constraints on the number of components that can be switched at a time. 
In these studies, the system becomes unstable (equivalent to the notion of permanent failure in our problem) if the state of a component violates any of the two interval thresholds. In contrast, our problem has one desirable threshold and one undesirable/failure threshold. Our problem is motivated by the fact that after shocks/disruptions, components such as infrastructure, infected servers, fire-affected regions etc., deteriorate rapidly in comparison to the deterioration faced during normal times. Thus, it can be assumed that the state of a component does not significantly varies due to normal deterioration processes once it is increased to full health and thus can be considered to be permanently repaired. Analogies to such a model can be found in control problems that use model predictive control where the aim is to stay in a set of desirable states and soft constraints are put on the set of undesirable states \cite{scokaert1999feasibility,mhaskar2006stabilization}. Soft constraints can be violated but a term is added in the objective function to penalize the violations. 
% The desirable and undesirable thresholds represent the health value of an infrastructure component when it is permanently repaired and permanently failed, respectively. 
%As mentioned before components can deteriorate to such a level after shocks/disruptions that they become unusable and require full replacement, which is expensive and thus undesirable. At that point, components can be considered to be \textit{permanently failed}.   
%This model is motivated by the fact that after disasters, infrastructure components such as roads and water/sewer pipes deteriorate rapidly in comparison to the deterioration faced during normal times. For instance, hairline cracks pose little threat to the functionality of pipes; however, in disasters, deterioration is accelerated until the cracks are repaired \cite{chisolm2012impact}. The structural strength of pavement sections submerged by floodwaters also significantly reduces over time \cite{sultana2014review}. Thus, it can be assumed that the health of a component does not significantly vary due to normal deterioration processes once it is repaired after disasters and thus can be considered to be \textit{permanently repaired}. Also, infrastructure components like pavement sections can deteriorate to such a level after disasters that they become unusable and require full replacement, which is expensive and thus undesirable \cite{sultana2016deterioration}. At that point, components can be considered to be \textit{permanently failed}. 
So, the objective of our problem is to maximize the weighted number of components whose states can be brought back to the desirable threshold value (or permanent repair) without ever reaching the undesirable threshold (permanent failure). This difference leads us to characterize optimal policies of different types depending on the problem conditions. We show that non-jumping policies, where switching between different components is not allowed until a component's state reaches full health, turn out to be optimal under some conditions. In contrast, the aforementioned studies related to switched systems do not characterize non-jumping policies to be optimal; indeed, jumping is necessary to meet the objectives of those problems.

Problems of a similar flavor can also be found in optimal control of robotic systems \cite{smith2012persistent} that persistently monitor changing environments; there, the goal is to keep the level of uncertainty about some dynamic phenomena below a certain threshold, with the uncertainty growing over time whenever the phenomenon is not being observed. Our problem also has similarities to the problem of allocating resources (e.g., time slots) at a base station to many time-varying competing flows/queues \cite{eryilmaz2007fair,eryilmaz2005stable,buche2004control}. However, these studies do not consider permanent failure of components or flows being serviced, and instead focus on either bounding the long-term state of the system, or maximizing long-term throughput or stability. Job scheduling problems with degrading processing times \cite{cheng2004concise,wei2012single,ng2010preemptive} as a function of job starting times also have analogies to our problem. A major difference between job scheduling and our problem is that in the former, a job is considered to be late if its \textit{completion} time exceeds the corresponding due date,  whereas in our problem, a component is considered to be failed if its health reaches the state of permanent failure before the entity \textit{starts} to control it. Another important difference is that a job is completely processed even if its completion time exceeds the corresponding due date; in contrast, a component cannot be fixed if its health value reaches the state of permanent failure.
%Most of these studies do not consider preemptive schedules (i.e., where one can jump from one job to another) and jobs are continuously fixed by the machine without any idle times between consecutive jobs. In contrast, in our study, time progresses in discrete time steps, capturing the resolution at which the entity makes decisions about which node to repair. 
Our problem also has similarities with scheduling analysis of real-time systems \cite{zhang2009schedulability}; there, the analysis focuses on real-time tasks that become available for processing at different times; in contrast, all the components in our problem are available for control starting at the same time. Patient triage scheduling problems \cite{argon2008scheduling} also have some analogies to our problem; these problems only focus on non-jumping sequences and characterize optimal sequences assuming that if a task has less time left before expiration than another task, then the former task also takes less time to be completed than the latter task. However, this assumption does not hold for the (non-jumping) policy that increases the state of the component that has the largest state at each time step that we characterize in this paper.   
%characterize optimal policies with equal and predefined deadlines for all jobs. %In contrast, the deadline (or the time of permanent failure) of an infrastructure component in our problem is a function of its health and the chosen repair sequence. 

In the conference version of this paper \cite{hgehlot2019optimal}, we studied the problem assuming that the rates of increase and decrease, and weights to be homogeneous across all the components. This paper significantly expands upon the conference paper by considering heterogeneous rates and weights, and showing that it is not optimal to switch away from a component before targeting it to full health when the decrease rates are larger than the increase rates (even for heterogeneous rates and weights across the components), and fully characterizing the optimal control policy when the rates of increase are sufficiently larger than the rates of decrease (even for heterogeneous rates and weights across the components).
The outline of the paper is as follows. In the next section, we formally present the problem that we consider in this paper. After this, we 
%first show that the general problem is NP-hard and then 
characterize the optimal control policies for some instances of this problem. Finally, we present the results of simulation studies to compare the optimal control policies with randomly generated control policies.    
